CERTainty: Detecting DNS Manipulation at Scale using TLS Certificates

DNS manipulation is an increasingly common technique used by censors and other network adversaries to prevent users from accessing restricted Internet resources and hijack their connections. Prior work in detecting DNS manipulation relies largely on comparing DNS resolutions with trusted control results to identify inconsistencies. However, the emergence of CDNs and other cloud providers practicing content localization and load balancing leads to these heuristics being inaccurate, paving the need for more verifiable signals of DNS manipulation. In this paper, we develop a new technique, CERTainty, that utilizes the widely established TLS certificate ecosystem to accurately detect DNS manipulation, and obtain more information about the adversaries performing such manipulation. We find that untrusted certificates, mismatching hostnames, and blockpages are powerful proxies for detecting DNS manipulation. Our results show that previous work using consistency-based heuristics is inaccurate, allowing for 72.45% false positives in the cases detected as DNS manipulation. Further, we identify 17 commercial DNS filtering products in 52 countries, including products such as SafeDNS, SkyDNS, and Fortinet, and identify the presence of 55 ASes in 26 countries that perform ISP-level DNS manipulation. We also identify 226 new blockpage clusters that are not covered by previous research. We are integrating techniques used by CERTainty into active measurement platforms to continuously and accurately monitor DNS manipulation.

==> blockpage.tex <==
\section{Generate \bp Fingerprints}
\label{sec:bp}
%\elisa{I want to express that \bp fingerprint generation is nothing new and is widely implemented, we've done a best-effort one}


 
Previous work have investigated different methods to identify \bps, utilizing clustering techniques based on the similarity of page length\cite{iclab, jones2014automated}, term frequency vectors\cite{jones2014automated}, HTML structure \cite{iclab} and the screenshot of the returned pages \cite{filtermap}.

All the mentioned \bp clustering techniques are followed by a step to manually create \bp fingerprints and appropriate labels for them. Constructing meaningful fingerprints is a widely accepted philosophy of \bp detection. Tedious as it seems, those \bp fingerprints provide valuable insights for the research community to track the scope, scale and evolution of content-based censorship. In this paper, we integrate publicly available \bp fingerprints \cite{cpbp} generated from application-layer blocking data \cite{filtermap}, and complementing it with more than 200 \bp fingerprints new generated from global DNS resolution data as one of the contribution of \platform. 

We clustered the returned pages based on page length and HTML structure. Jones \etal reported that the page length similarity works best with tuned threshold, resulting in 95\% true positive rate and 1.37\% false positive rate \cite{jones2014automated}. We observed the same pattern and conclude that page length works best. %Different from previous work which is domain-centric \cite{jones2014automated, iclub}, \ie clustering based on the insight that 
%\elisa{Ask Ram: I don't want to spend too many words describing our slightly different method - from domain-centric to ip-centric, taking status code into account, etc. Do we want to talk about the page element based clustering helps us to find pages with variable name that have "internet health" in it, which will be difficult for image clustering?}

\input{table/bp_fingerprint}
We  manually verified each blockpage cluster is in order to remove false positives. The presence of \bps are relatively stable in our dataset. For over 3 month's time (from March, 2022 to June, 2022), only 13 new potential cluster is observed. Therefore  the manual efforts for generating \bp fingerprints is minimized.  We crafted the \bp fingeprints into 6 categories as it is shown in Table \ref{table:fp_dist}, following the convention set by previous work done by R. Sundara Raman \etal \cite{filtermap} as it is shown in Table~\ref{table:fp_dist}:
\begin{itemize}
    \item \textbf{Commercial product}: commercial middleboxes \eg OpenDNS \cite{contreras_2022}, NextDNS\cite{nextdns}, OneDNS \cite{onedns}, Zxyel \cite{zxyel}. %\elisa{do we want to do things similar to the filtermap country map for commercial products?}
    \item  \textbf{National-level \dnscensorship}: \eg Indonesia \bps that have "Internet Positif (Positive Internet)" in the webpage.
    \item \textbf{ISP-specific \bps}: \eg Fig. \ref{fig:rubp}.
    \item \textbf{Corporational or institutional \dnscensorship}: \eg companies and universities. 
    \item \textbf{Unknown}: \bps that we do not have enough information to attribute their origin. Each such fingerprint is annotated with the country where the IPs which host the blockpages are from.
    \item \textbf{General}:  \eg "This Site Has Been Blocked" in the HTML title.
    
\end{itemize}

We use the fingerprint to conduct health check for control resolvers, allowing future control resolver list expansion. We open-source the annotated fingerpints for the community. The \bp fingerprint is also used as the ground truth to justify using certificate validation in \S\ref{sec:cert}



==> dead.tex <==
% \subsection{Determine the Validity of Certificates}
% For a given certificate chain, we call it \textit{valid} if all the following conditions are satisfied:
% %\deepak{I would swap 1) and 2)}
% \begin{enumerate}
%     \item \textit{Correct and Trusted Certificate}: The certificate chain is corrected signed and trusted by major browsers.
%     \begin{enumerate}
%         \item \textit{Correctly Signed Certificate Chain}: \platform uses OpenSSL \cite{openssl} to verify the certificate chains.% \elisa{Ask Deepak: word choice}. \deepak{Verify the certificate chains to a trusted root is probably good enough.}
%         \item \textit{Trusted Root Certificate}: for \platform, we are using Certifi\cite{certifi} to verify the chain to a trusted root. Certifi is Mozilla's curated collection of root Certificates.
%     \end{enumerate}
    
%     \item \textit{Hostname Matching}: The domain name matches with the hostname in the leaf certificate \ie at least one of the following conditions is satisfied:
%     \begin{enumerate}
%         \item The hostname exactly matches the Common Name in the certificate's Subject.
%         \item The hostname is listed in the Subject Alternative Name field or  matches a wild card in the Alternative Name field.
%         \item For special cases \eg traditional domain names and internationalized domain names, we follow the rules as it is specified in RFC 6125 \cite{certhostname}.
%     \end{enumerate}
% \end{enumerate}


\subsection{Tolerating Test Certificate Misissurance}
In order to further exclude invalid certificates because of misconfiguration, \platform incorporates the following \metrics for certificate validation:

\paragraph{Tolerating misissuance of deprecated root certificates} 
We see about 3.6\% of the all certificate chains that violate condition 2-a) "Correctly Signed Certificate Chain" but have at least one certificate in the chain trusted by Certifi\cite{certifi}. Upon further investigation, more than 86\% of them are issued by Let's Encrypt\cite{letsencrypt} and see a DST Root CA, which is deprecated by Let's Encrypted on September 30, 2021, but a small percentage of this root certificate is still lingering on the Internet\cite{dst}. When checking the HTML pages returned along with the certificate, they are expected pages for the requested domains. Therefore, we still consider such a chain of certificates is valid if there exist a sub chain that is both verified by Certifi to a trusted root and correctly signed.

\paragraph{Tolerating misissuance of shortly expired certificates} About 0.47\% unique certificate chains failed condition 1-a) "Correctly Signed Certificate Chain" because an expired leaf certificate or an intermediate certificate. For the ones that have a trusted root and matching hostname, and expired in less than 5 days as of the measurement time, we still view the chain as correctly signed. Note that the tolerating mechanism is only for the correctness and trustworthiness of the chain and will not affect the outcome of hostname matching.






\subsection{Construct Control Pool}
%\deepak{Explain first what your high level goals are. For example: ``we use certificate validity as a proxy for determining censorship. In order to do this, we need to first set up a pool of controls, which will serve as ground truth for the case where no censorship occurs.''}

Invalid certificates are not rare on the Internet \cite{ukrop2019will, kumar2018tracking, akhawe2013here, acer2017wild}. To use certificate validity as a proxy for detecting \dnscensorship, we need to set up a pool of controls that serves as ground truth for the case where the certificates are invalid because of deployment errors/misconfiguration from domain administrators.  For simplicity we use \textit{control certificate} to denote a certificate returned by a IP from a control resolver's resolution and \textit{test certificate} to denote a certificate returned by a IP from a test resolver's resolution.

We see 1.2\% to 1.3\%  invalid certificates among all unique control certificates collected, representing 3.24\% of the 2,000 domains in \platform's test list. This means the certificates for those domains are not issued correctly by default and the presence of invalid certificates for those domains are not necessarily a signal of \dnscensorship.  Fig. \ref{fig:invalid_ctrl_cert} contains 3 examples of the invalid control certificates.  We see a good proportion of .mil and .gov domains failing certificate validation such as \code{www.dtic.mil}, which confirms statistics provided in prior works \cite{acer2017wild}. The US goverment and military websites are using a different PKI called Federal PKI, which is not a publicly trusted certificate authority \cite{govcert}. Other misconfigured domains \eg \code{www.freeexpression.org} and \code{www.kcna.kp} either have invalid certificates because of mismatching hostname, or untrusted root CA. When examining the test certificates, we tag the invalid certificates that are compatible with an invalid certificate as \code{unmanipulated/malformed\_domain} and do not consider it as a signal of \dnscensorship. 

%\elisa{to have a CDF of the amount of different point of presense of domains?}.

%\deepak{You might want to signpost better here - what do the four cases mean? Why are you splitting things into four cases?}

We consider the presence of a \bp to be solid indication that an IP hosting an invalid certificate is manipulated. When no \bps are served, we check additional information \eg certificate common name, subject alternative name and issuer \cite{certhostname}. If the certificate is issued by a known TLS proxy vendor or an ISP, we consider it evidence of true \dnscensorship signal.

In the following sections, we will investigate the four cases of certificate validity based on hostname matching and trusted root. Through the in-depth analysis we establish confidence of using certificate validity as a proxy to detect \dnscensorship, through \bp fingerprint matching and manual analysis.

%\will{would be useful to have the decision tree diagram you've been using to organize cases as a visual representation of taxonomy of outcomes.} 



%None of the HTML pages returned with a valid certificate matches any \bp fingerprint. Some CDNs would return HTTP(S) pages with client error status code since our measurement machine is not in their costumer IPs. However, in this case the correct certificates for the requested domains are still returned. Therefore, certificate validation can not only signal the correctness of DNS resolution when an expected page is served, but also transcend the limitations of geoblocking based on the remote measurement vantage point location.

.
We plot the distribution of \bp fingerprint matching and invalid control certificate matching  based on the HTTP status code returned with the test certificates in Fig.~\ref{fig:match_untrusted_cert}-(1). The HTTP status code contains information of the returned pages:
\begin{enumerate}
    \item \textit{Successful status code}: either the correct page or \bp of the queried domain is returned.
    \item \textit{Redirect status code}: either redirecting user to the correct resource, or redirecting to a \bp.
    \item \textit{Client error status code}: including 400 Bad Request, 403 Forbidden, 404 Not Found, and 451 Unavailable For Legal Reasons.
    \item \textit{Server error status code}: the server is not able to handle the request.
\end{enumerate}


We do not see such misconfigured certificates in the control pool. In a user's perspective, if such a misconfigured IP is returned, the user will not be able to access the desired content. Therefore we view this as a case of \dnscensorship as well. %\elisa{should we go there?}




%Table~\ref{tab:previous_work} summarizes previous work on \dnscensorship detection when public IPs are returned, comparing to \platform. We omit country-specific detection \metrics designed based on the behavior of national firewall \eg the GFWatch \cite{greatgfw}, which trigger Chinese middleboxes by sending DNS queries across border to self-own machines without DNS resolution capacities, as well as Aryan \etal that checks if the Iranian resolvers return private IPs \cite{alexiran}.

%In this section, we discuss why the previous \metrics under the independent verifiability \cat are not properly designed. We also demonstrate that despite being intuitive, the consistency \cat introduces both false positives and false negatives into the system. 


% \label{sec:consistency}
% As shown in Table~\ref{tab:previous_work}, all the platforms mentioned in Table~\ref{tab:previous_work} incorporate a ``test vs control'' strategy---comparing the DNS resolution with resolution from a set of trusted resolvers---and mostly focus on identifying correct resolution through the consistency of returned IPs and their metadata. The \metrics under the consistency \cat were developed based on the insight that, behind the same domain name, there are some shared infrastructural services. Alternatively, some work leverage fine-tuned statistical threshold for domain mapping to the same IP, or the TTL field in the DNS packets. Different platforms have incorporated a wide range of extra data to increase the capacity to recognize unmanipulated DNS responses because control IP matching cannot fully cover all correct PoPs of queried domains.

% \iris \cite{iris} leverages the metadata of resolved IPs: Autonomous System (AS) number and name, HTTP content hash, HTTPS certificate hash, and PTRs. If the IP or \textit{any} of the metadata matches with the control group, the DNS response is tagged as unmanipulated. The HTTP content hash and HTTPS certificate hash are not independent verifiability \metrics since all the information above is added through an additional tagging stage, using metadata from Censys\cite{censyspaper} and Maxmind\cite{maxmind}. The effectiveness of each \metric reported by \iris is shown in Table~\ref{tab:iris_res}. %\eg AS number, AS name, HTTP content hash and HTTPS certificate hash



%\iris reported poor performance of the independent verifiability \metrics. As shown in Table \ref{tab:iris_res}, the correct certificate \metrics are only able to identify 40\% to 70\% of the unmanipulated responses, while the same AS \metric can identify more than 90\% of the unmanipulated responses. 

%UBICA \cite{aceto2015monitoring} utilizes page size to identify \dnscensorship. Using the information of fetched pages is good intuition, though naively comparing the size with control groups will not yield meaningful results since a lot of websites host different contents based on user geolocation. \platform takes this idea a step further by extracting page information such as page length and HTML structure to cluster potential \bps, producing expert-curated fingerprints to identify the actors behind \dnscensorship. 
 
%For the case of certificate with SNI specified, \iris checks whether the certificate returned is  a valid, browser-trusted certificate for the correct \textit{IP address}, instead of the queried domain, which could be another source of false positives.



\subsection{Designing Evaluation Metrics}
%\elisa{maybe we can just delete the following paragraph?}
%\iris used the ability to identify unmanipulated responses to quantify the effectiveness of different \metrics \cite{iris}. The effectiveness of  each \metric to identify unmanipulated responses is shown in Table \ref{tab:iris_res}. The unmanipulated responses in \iris is defined as the responses which pass at least one of the aforementioned \metric. Therefore this evaluation metric is more qualitative than quantitative.

\dnscensorship is rare on the global scale. Previous work reported 2\% to 4\%  \dnscensorship rate when conducting global measurement \cite{iris, censoredplanet, dagon2008corrupted}. Therefore, we do not have confidence on a \metric even if it comes with 90\% accuracy of identifying \textit{unmanipulated} responses, since it is still over reporting \dnscensorship by a significant margin. Instead, properly designed detection \metrics should actively look for signals of \dnscensorship. It is also hard to construct a set of \textit{ground truth}. For a single snapshot, more than 40 million lines of DNS resolution are recorded, making it impossible for us to manually verify and construct a complete set of (un)manipulated responses. However, through the lens of the cross-checking the results of the consistency \metric and \platform, we have a good understanding of effectiveness of the consistency \metrics.

Because \iris covers all consistency \metrics previously purposed except the threshold and TTL method, we view it as the state-of-the-art and conduct comparison between our results with \iris's consistency \cat. Censored Planet's DNS measurement platform \cite{censoredplanet} inherited the consistency \metrics from \iris and has been releasing data since 2018. We cross-check two measurement platform's results using Censored Planet's open source data.

%\paragraph{IP, HTTP Hash and Certificate Hash Matching}
%The presence of control-matching IP, HTTP hash and certificate hash is a strong signal of correct resolution. However, the latter two are are tightly associated the the presence of control-matching IPs (90.05\% and 83.08\% respectively). For the HTTP hash matching without control IP matching, we see a majority of error HTTP page matching (with 403 or 404 status code), which does not serve the purpose of confirming the correctness of DNS resolution. We see the same outcome for certificate hash, the control-matching certificate hash without IP matching are mostly general CDN certificates---this again demonstrate the importance of requesting certificates with SNI.


==> fig_tex/anno_dt.tex <==
\begin{figure}[t] 
 \centering
 \includegraphics[width=0.99\columnwidth]{figure/dt_anno.pdf}
 \caption{Decision tree of \platform's write back heuristic}
\label{fig:ann_dt}
\end{figure}

==> fig_tex/arch.tex <==
\begin{figure*}[t] 
 \centering
 \includegraphics[width=1.99\columnwidth]{figure/arch.pdf}
 \caption{\textbf{\platform Pipeline}--- This picture needs to be re-done.}
\label{fig:arch}
\end{figure*}

%\platform generates a list of domains for DNS resolution, as well as a list of ethical global open resolvers and trusted control resolvers. (2) DNS queries for the domains are sent to global resolvers. (3) HTTP(S) page requests are sent to IPs returned by test resolvers and control resolvers. (4) Returned DNS responses and HTTP(S) page responses are fed into \platform's DNS manipulation identification pipeline. (5) Generated \bp fingerprints as well as annotated DNS data are published to the public.

==> fig_tex/domains_pop.tex <==
\begin{figure}[t] 
 \centering
 \includegraphics[width=0.99\columnwidth]{figure/domains_pop.pdf}
 \caption{\textbf{Number of country with at least one PoP}---for all the domains in \platform's test list.}
\label{fig:domains_pop}
\end{figure}

==> fig_tex/gamban.tex <==
\begin{figure}[!t]
 \centering
    \includegraphics[scale=0.2]{figure/gamban.png}
    \caption{\textbf{Filtering services utilizing non-zero \rcode}---Gamban website introducing its blocking services, which we discover by investigating \code{RCODE:3}}
    \label{fig:gamban}
\end{figure}

==> fig_tex/invalid_ctrl_cert.tex <==
\begin{figure}
\centering
    \includegraphics[width=\columnwidth]{figure/invalid_ctrl_certs.png}
    \caption{\textbf{Error messages of invalid control certificates collected by \platform}---(1) Certificate for https://dtic.mil/ (2) Certificate for https://www.freeexpression.org/ (3) Certificate for https://www.kcna.kp/.}
    \label{fig:invalid_ctrl_cert}
\end{figure}

==> table/iris_res.tex <==
\begin{table}[t]
    %\scriptsize
    \small
    \centering
    \begin{tabular}{m{4em} m{1em} m{1.8em} m{1em} m{1em} m{1em} m{1em} m{1em} m{5em}}
    \toprule
    {} & {} & {} & {Consistency} & {} & {} &{} &{Ind.} &{ Verifiability} \\
    {Heuristics} & {IP} & {HTTP hash} & {Cert hash} & {AS} & {CDN} & {} & {Cert} & {Cert w/ SNI}\\ 
    \midrule
    {About} & {90\%} & {$ 80\%$} & {$ 75\%$} & {$ 95\%$} & {$ 10\%$} & {} & {$ 40\%$} & {$ 70\%$} \\     
    \bottomrule
    \end{tabular}
    \caption{\textbf{Consistency \metrics effectiveness}---Effectiveness of different \metrics on identifying unmanipulated responses reported in \protect\cite{iris}-Figure 3. }
    \label{tab:iris_res}
\end{table}

==> table/removed_noises.tex <==
% \begin{table}[ht!]
% \centering
% \begin{tabular}{|p{8mm} p{13mm} p{19mm} p{10mm} p{12mm} |} 
%  \hline
%  \textbf{Category} & \textbf{Liveness} & \textbf{Timeout} & \textbf{\rcode} & \textbf{Zero IPs}  \\ 
%  \hline
%  \textbf{Count} & 1457323 & 0 & 116500? & 0 \\ 
%  \hline
%  \hline
%   \xspace & \textbf{Private IPs} & \textbf{Captive Portals} & \textbf{Original} & \textbf{Filtered}\\
%  \hline
%  \textbf{Count} &  0 & 680512 & 50090223 & ? \\
%  \hline
% \end{tabular}
% \caption{Statistics on the percentage of filtered responses}
% \label{table:remove_broken}
% \end{table}

\begin{table}[ht!]
\small
\caption{Statistics on the percentage of filtered responses}
\label{table:remove_broken}
\centering
\begin{tabular}{p{8mm} p{13mm} p{19mm} p{10mm} p{12mm}} 
 \toprule
 \textbf{Category} & \textbf{Liveness} & \textbf{Timeout} & \textbf{\rcode} & \textbf{Zero IPs}  \\ 
 \midrule
 \textbf{Count} & 1,457,323 & 0 & 116,500? & 0 \\ 
 \midrule
  \xspace & \textbf{Private IPs} & \textbf{Captive Portals} & \textbf{Original} & \textbf{Filtered}\\
 \midrule
 \textbf{Count} &  0 & 680,512 & 50,090,223 & ? \\
 \bottomrule
\end{tabular}
\end{table}
